Data-Driven Robust Taxi Dispatch under Demand Uncertainties

In modern taxi networks, large amounts of taxi occupancy status and location data are collected from networked in-vehicle sensors in real-time. They provide knowledge of system models on passenger demand and mobility patterns for efficient taxi dispatch and coordination strategies. Such approaches face new challenges: how to deal with uncertainties of predicted customer demand while fulfilling the system's performance requirements, including minimizing taxis' total idle mileage and maintaining service fairness across the whole city; how to formulate a computationally tractable problem. To address this problem, we develop a data-driven robust taxi dispatch framework to consider spatial-temporally correlated demand uncertainties. The robust vehicle dispatch problem we formulate is concave in the uncertain demand and convex in the decision variables. Uncertainty sets of random demand vectors are constructed from data based on theories in hypothesis testing, and provide a desired probabilistic guarantee level for the performance of robust taxi dispatch solutions. We prove equivalent computationally tractable forms of the robust dispatch problem using the minimax theorem and strong duality. Evaluations on four years of taxi trip data for New York City show that by selecting a probabilistic guarantee level at 75%, the average demand-supply ratio error is reduced by 31.7%, and the average total idle driving distance is reduced by 10.13% or about 20 million miles annually, compared with non-robust dispatch solutions.

==> bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1in,clip,keepaspectratio]{bio/feimiao.jpg}}]{Fei Miao} (S'13-M'16) is an Assistant Professor in the Department of Computer Science and Engineering at the University of Connecticut. Previously, she was a Postdoc Researcher in the Department of Electrical and Systems Engineering, GRASP Lab and PRECISE center, at the University of Pennsylvania. She received the B.Sc. degree in Automation from Shanghai Jiao Tong University in 2010,  the M.A. degree in Statistics and the Ph.D. degree with the "Charles Hallac and Sarah Keil Wolf Award for Best Doctoral Dissertation" in Electrical and Systems Engineering from the University of Pennsylvania in 2015 and 2016, respectively. Her research interests include data-driven real-time optimization and control of cyber-physical systems under model uncertainties, and resilient and secure control cyber-physical systems. She was a Best Paper Award Finalist at the 6th ACM/IEEE International Conference on Cyber-Physical Systems in 2015.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/shuohan.jpg}}]{Shuo Han}  (S'08-M'14) is an Assistant Professor in the Department of Electrical and Computer Engineering at the University of Illinois at Chicago (UIC). Previously, he was a postdoctoral researcher in the Department of Electrical and Systems Engineering at the University of Pennsylvania. He received his B.E. and M.E. in Electronic Engineering from Tsinghua University in 2003 and 2006, and his Ph.D. in Electrical Engineering from the California Institute of Technology in 2013. His current research focuses on developing rigorous frameworks for data-driven decision making that enable reliable and efficient operations of networked cyber-physical systems, including many smart city applications such as power and transportation networks. He was a finalist for the Best Student Paper Award at the 2013 American Control Conference.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/shanlin.jpg}}]{Dr. Shan Lin} is an assistant professor of the Electrical and Computer Engineering Department at Stony Brook University. He received his PhD in computer science at the University of Virginia in 2010. His PhD dissertation is on Taming Networking Challenges with Feedback Control. His research is in the area of networked systems, with an emphasis on feedback control based design for cyber-physical systems and sensor systems. He works on wireless network protocols, interoperable medical devices, smart transportation systems, and intelligent sensing systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/QianWang.jpg}}] {Qian Wang} has been serving product and strategy leadership roles in
multiple financial technology firms in Asia, including Advance.AI, a
fintech company mainly serving South East Asia, and China Chengxin
Credit Information, one of the leading credit data service providers
in China. Previously, he worked on scalable and high performance data
platforms at Two Sigma Investments, a quantitative hedge fund
headquartered in New York. Qian Wang graduated from the University of
Pennsylvania with a bachelor's degree and a master's degree, both in
Computer and Information Science.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/jackstankovic.jpg}}]{Professor John A. Stankovic} is the BP America Professor in the Computer Science Department at the University of Virginia. He is a Fellow of both the IEEE and the ACM. He has been awarded an Honorary Doctorate from the University of York. He won the IEEE Real-Time Systems Technical Committee's Award for Outstanding Technical Contributions and Leadership.  He also won the IEEE Technical Committee on Distributed Processing's Distinguished Achievement Award. He has seven Best Paper awards, including one for ACM SenSys 2006. Stankovic has an h-index of 105 and over 40,000 citations. Prof. Stankovic received his PhD from Brown University.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/Hendawi.jpg}}] {}Abdeltawab Hendawi} is a Postdoc Research Associate in Computer Science at the University of Virginia. He completed his MSc and PhD in Computer Science and Engineering from the University of Minnesota, Twin Cities, 2012 and 2015 respectively. His research interests are centered on data management and analysis with more focus on smart cities related applications. His work has been recognized by a number of awards, including the Best Paper Award at the ACM SIGSPATIAL MobiGIS 2012, the Best Poster Award at the U-Spatial Symposium 2013; the Best Demo Paper Awards at the ACM SIGSPATIAL 2014 and at the IEEE MDM 2015. Dr. Hendawi’s vision for smart location-aware services in smart cities also won a highly recognized Award, blue sky ideas award 2016.  In addition, Dr. Hendawi is the recipient of the Hobby postdoctoral Research Fellowship 2015-2018 from the Computer Science Department at the University of Virginia.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/Deszhang.jpg}}]{Desheng Zhang} Desheng is an assistant professor at the Department of Computer Science at Rutgers University. Desheng is broadly concentrated on bridging cyber-physical systems and big urban data by technical integration of communication, computation, and control in data-intensive urban systems. He is focused on the life cycle of big-data-driven urban systems, from multi-source data collection to streaming-data processing, heterogeneous-data management, model abstraction, visualization, privacy, service design and deployment in complex urban settings. Desheng is currently interested in real-time interactions among heterogeneous urban systems including cellphone, smartcard, taxi, bus, truck, subway, bike, personal vehicle, electric vehicle, and road networks. He is a member of IEEE.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/tianhe1.jpg}}]{Dr. Tian He} is currently an associate professor in the Department of Computer Science and Engineering at the University of Minnesota-Twin City. Dr. He is the author and co-author of over 200 papers in premier network journals and conferences with over 17,000 citations (H-Index 52). Dr. He is the recipient of the NSF CAREER Award, George W. Taylor Distinguished Research Award and McKnight Land-Grant Professorship, and many best paper awards in networking.  His research includes wireless sensor networks, cyber-physical systems, intelligent transportation systems, real-time embedded systems and distributed systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/GJpappas.jpg}}]{George J. Pappas} (S'90-M'91-SM'04-F'09) received the Ph.D. degree in electrical engineering and computer sciences from the University of California, Berkeley, CA, USA, in 1998. He is currently the Joseph Moore Professor and Chair of the Department of Electrical and Systems Engineering, University of Pennsylvania, Philadelphia, PA, USA. He also holds a secondary appointment with the Department of Computer and Information Sciences and the Department of Mechanical Engineering and Applied Mechanics. He is a Member of the GRASP Lab and the PRECISE Center. He had previously served as the Deputy Dean for Research with the School of Engineering and Applied Science. His research interests include control theory and, in particular, hybrid systems, embedded systems, cyber-physical systems, and hierarchical and distributed control systems, with applications to unmanned aerial vehicles, distributed robotics, green buildings, and bimolecular networks. Dr. Pappas has received various awards, such as the Antonio Ruberti Young Researcher Prize, the George S. Axelby Award, the Hugo Schuck Best Paper Award, the George H. Heilmeier Award, the National Science Foundation PECASE award and numerous best student papers awards at ACC, CDC, and ICCPS.
\end{IEEEbiography}



